QED$_3$ with quenched disorder: quantum critical states with interactions and disorder

Quantum electrodynamics in 2+1-dimensions (QED$_3$) is a strongly coupled conformal field theory (CFT) of a U(1) gauge field coupled to $2N$ two-component massless fermions. The $N=2$ CFT has been proposed as a ground state of the spin-1/2 kagome Heisenberg antiferromagnet. We study QED$_3$ in the presence of weak quenched disorder in its two spatial directions. When the disorder explicitly breaks the fermion flavor symmetry from SU($2N$)$\rightarrow$U(1)$\times$SU($N$) but preserves time-reversal symmetry, we find that the theory flows to a non-trivial fixed line at non-zero disorder with a continuously varying dynamical critical exponent $z>1$. We determine the zero-temperature flavor (spin) conductivity along the critical line. Our calculations are performed in the large-$N$ limit, and the disorder is handled using the replica method.

==> 4points.tex <==
\centering
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
\begin{fmffile}{4pts1}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2a}
\fmf{dashes}{v1b,v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}
\end{fmffile}}
\notag}
%\vspace{8mm}
\caption{}
\label{fig:4ptSigmaSigmaNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
\begin{fmffile}{4pts2}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2b}
\fmf{dashes}{v1b,v2a}
%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}
\end{fmffile}}
\notag}
\caption{}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
\begin{fmffile}{4pts3}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1c,v2c}
\fmf{dashes,left,tension=0}{v1a,v1b}
%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}
\end{fmffile}}
\notag}
\caption{}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{15mm}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
\begin{fmffile}{4pts4}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2a}
\fmf{dashes}{v1b,v2b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2a}
%\fmfkeep{suscept}
\end{fmfgraph*}
\end{fmffile}}
\notag}
\caption{}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
\begin{fmffile}{4pts5}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2b}
\fmf{dashes}{v1b,v2a}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2b}
\end{fmfgraph*}
\end{fmffile}}
\notag}
\caption{}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
\begin{fmffile}{4pts6}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1c,v2c}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v1b}
\fmf{dbl_dashes,left,tension=0}{v1a,v1b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v1b}
%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}
\end{fmffile}}
\notag}
\caption{}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{15mm}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
%\begin{fmffile}{4pts7}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2a}
\fmf{dbl_dashes}{v1b,v2b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2a}
\fmfv{l=$b$}{v1b}
\fmfv{l=$b$}{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}
%\end{fmffile}
}
\notag}
\caption{}
\label{fig:4ptPhiPhiNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
%\begin{fmffile}{4pts8}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2b}
\fmf{dbl_dashes}{v1b,v2a}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2b}
\fmfv{l=$b$}{v1b}
\fmfv{l=$b$}{v2a}
\end{fmfgraph*}
%\end{fmffile}
}
\notag}
\caption{}
\label{fig:4ptPhiPhiX}
\end{subfigure}
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
\begin{fmffile}{4pts9}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v1b}
\fmf{dbl_dashes,left,tension=0}{v1a,v1b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v1b}
\fmfv{l=$b$}{v1c}
\fmfv{l=$b$}{v2c}
%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}
\end{fmffile}}
\notag}
\caption{}
\label{fig:PhiPhiVert}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{15mm}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.32\textwidth}
\eq{
\mff{
\begin{fmffile}{4pts10}
\small
\begin{fmfgraph*}(40,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v1b}
\fmf{dashes,left,tension=0}{v1a,v1b}
\fmfv{l=$a$}{v1c}
\fmfv{l=$a$}{v2c}
%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}
\end{fmffile}}
\notag}
\caption{}
\label{fig:PhiPhiVert}
\end{subfigure}













%\begin{figure}[h]
%\centering
%\begin{subfigure}[b]{0.32\textwidth}
%\eq{
%\mff{
%\begin{fmffile}{4pts1}
%\small
%\begin{fmfgraph*}(40,20)
%\fmfpen{thin}
%\fmfstraight
%\fmfleft{i2,i1}
%\fmfright{o2,o1}
%%\fmflabel{$\mu$}{i1}
%%\fmf{phantom,tension=2}{i1,o1}
%%\fmffreeze
%\fmf{phantom}{i1,v1a}
%\fmf{phantom}{i2,v2a}
%\fmf{phantom,tension=.6}{v1a,v1b}
%\fmf{phantom,tension=.6}{v2a,v2b}
%\fmf{phantom}{v1b,o1}
%\fmf{phantom}{v2b,o2}
%\fmffreeze
%\fmf{fermion,label=$(s-1)p$,label.side=left}{i1,v1a}
%\fmf{fermion,label=$-q+sp$,label.side=right}{v1a,v1b}
%\fmf{fermion}{v1b,o1}
%\fmf{fermion,label=$p$}{i2,v2a}
%\fmf{fermion,label=$q+p$}{v2a,v2b}
%\fmf{fermion,label=$sp$}{v2b,o2}
%\fmf{dashes,label=$q-p$}{v1a,v2a}
%\fmf{dashes,label=$q+(1-s)p$,label.side=left}{v1b,v2b}
%%\fmfkeep{suscept}
%\end{fmfgraph*}
%\end{fmffile}}
%\notag}
%\vspace{8mm}
%\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}[b]{0.32\textwidth}
%\eq{
%\mff{
%\begin{fmffile}{4pts2}
%\small
%\begin{fmfgraph*}(40,20)
%\fmfpen{thin}
%\fmfstraight
%\fmfleft{i2,i1}
%\fmfright{o2,o1}
%%\fmflabel{$\mu$}{i1}
%%\fmf{phantom,tension=2}{i1,o1}
%%\fmffreeze
%\fmf{phantom}{i1,v1a}
%\fmf{phantom}{i2,v2a}
%\fmf{phantom,tension=.6}{v1a,v1b}
%\fmf{phantom,tension=.6}{v2a,v2b}
%\fmf{phantom}{v1b,o1}
%\fmf{phantom}{v2b,o2}
%\fmffreeze
%\fmf{fermion,label=$(s-1)p$,label.side=left}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
%\fmf{fermion}{v1b,o1}
%\fmf{fermion,label=$p$}{i2,v2a}
%\fmf{fermion,label=$q+p$}{v2a,v2b}
%\fmf{fermion,label=$sp$}{v2b,o2}
%\fmf{dashes}{v1a,v2b}
%\fmf{dashes}{v1b,v2a}
%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%%\fmfkeep{suscept}
%\end{fmfgraph*}
%\end{fmffile}}
%\notag}
%\vspace{8mm}
%\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}[b]{0.32\textwidth}
%\eq{
%\mff{
%\begin{fmffile}{4pts3}
%\small
%\begin{fmfgraph*}(40,20)
%\fmfpen{thin}
%\fmfstraight
%\fmfleft{i2,i1}
%\fmfright{o2,o1}
%%\fmflabel{$\mu$}{i1}
%%\fmf{phantom,tension=2}{i1,o1}
%%\fmffreeze
%\fmf{phantom}{i1,v1a}
%\fmf{phantom}{i2,v2a}
%\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
%\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
%\fmf{phantom}{v1b,o1}
%\fmf{phantom}{v2b,o2}
%\fmffreeze
%\fmf{fermion,label=$(s-1)p$,label.side=right}{i1,v1a}
%%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
%\fmf{fermion}{v1a,v1c}
%\fmf{fermion}{v1c,v1b}
%\fmf{fermion}{v1b,o1}
%\fmf{fermion,label=$p$}{i2,v2c}
%\fmf{fermion,label=$sp$}{v2c,o2}
%\fmf{dashes}{v1c,v2c}
%\fmf{dashes,left,tension=0}{v1a,v1b}
%%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%%\fmfkeep{suscept}
%\end{fmfgraph*}
%\end{fmffile}}
%\notag}
%\vspace{8mm}
%\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%\hspace{10mm}
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%\caption{4-points}
%\end{figure}

==> 4pointsChiChi00.tex <==
\centering
\begin{fmffile}{4ptsChiChi00}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_wiggly}{v1a,v2a}
\fmf{dbl_wiggly}{v1b,v2b}
\fmfv{l=$b,,0$}{v1a}
\fmfv{l=$b,,0$}{v2a}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
\caption{$
\sum_{ab}{g_{v,a}g_{v,b}\o4\pi\ep}\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]+
\sum_a\(-{g_{v,a}^2\o4\pi\ep}\)\[\g^j\otimes\g_j\]\[\id\otimes\id\]$}
%\label{fig:4ptSigmaSigmaNoX}
\label{fig:4ptChiChi00NoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_wiggly}{v1a,v2b}
\fmf{dbl_wiggly}{v1b,v2a}
\fmfv{l=$b,,0$}{v1a}
\fmfv{l=$b,,0$}{v2b}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\caption{$
\sum_{ab}{g_{v,a}g_{v,b}\o4\pi\ep}\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]+
\sum_a\({g_{v,a}^2\o4\pi\ep}\)\[\g^j\otimes\g_j\]\[\id\otimes\id\]$}
%\label{fig:4ptSigmaSigmaX}
\label{fig:4ptChiChi00X}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\
\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_wiggly}{v1c,v2c}
\fmf{dbl_wiggly,left,tension=0}{v1a,v1b}
\fmfv{l=$b,,0$}{v1b}
\fmfv{l=$b,,0$}{v1a}
\fmfv{l=$a$,l.a=-55}{v1c}
\fmfv{l=$a$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$a,,0$,l.a=-55}{v1c}
\fmfv{l=$a,,0$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(-{g_{v,a}\o\pi\ep}\)\(2g_{v,a}-\sum_bg_{v,b}\)\[\g^0\otimes\g^0\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_wiggly}{v1c,v2c}
\fmf{photon,left,tension=0}{v1a,v1b}
\fmfv{l=$\m$}{v1b}
\fmfv{l=$\m$}{v1a}
\fmfv{l=$a$,l.a=-55}{v1c}
\fmfv{l=$a$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$a,,0$,l.a=-55}{v1c}
\fmfv{l=$a,,0$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(-{16g_{v,a}\mathpzc{g}^2\o3\pi^2(2N)\ep}\)\[\g^0\otimes\g^0\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}

==> 4pointsChiChiX0.tex <==
\centering
\begin{fmffile}{4ptsChiChiX0}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_plain}{v1a,v2a}
\fmf{dbl_wiggly}{v1b,v2b}
\fmfv{l=$b,,j$}{v1a}
\fmfv{l=$b,,j$}{v2a}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
\caption{
$\sum_a{g_{v,a}g_{\A,a}\o\pi\ep}\bigg\{-\[\id\otimes\id\]\[\id\otimes\id\]$
$+\[\g^0\otimes\g^0\]\[\id\otimes\id\]\bigg\}$
$+\sum_{ab}{g_{v,a}g_{\A,b}\o\pi\ep}\sum_c\abs{\ep^{abc}}\bigg\{
\[\id\otimes\id\]\[\s_c\otimes\s_c\]$
$-\[\g^0\otimes\g^0\]\[\s_c\otimes\s_c\]\bigg\}
$}
\label{fig:4ptChi0ChiXNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_plain}{v1a,v2b}
\fmf{dbl_wiggly}{v1b,v2a}
\fmfv{l=$b,,j$}{v1a}
\fmfv{l=$b,,j$}{v2b}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\caption{
$\sum_a{g_{v,a}g_{\A,a}\o\pi\ep}\bigg\{-\[\id\otimes\id\]\[\id\otimes\id\]$
$-\[\g^0\otimes\g^0\]\[\id\otimes\id\]\bigg\}$
$+\sum_{ab}{g_{v,a}g_{\A,b}\o\pi\ep}\sum_c\abs{\ep^{abc}}\bigg\{$
$-\[\id\otimes\id\]\[\s_c\otimes\s_c\]$
$-\[\g^0\otimes\g^0\]\[\s_c\otimes\s_c\]\bigg\}
$}
\label{fig:4ptChi0ChiXX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.6\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_wiggly}{v1c,v2c}
\fmf{dbl_plain,left,tension=0}{v1a,v1b}
\fmfv{l=$b,,j$}{v1b}
\fmfv{l=$b,,j$}{v1a}
%\fmfv{l=$a,,j$,l.a=-55}{v1c}
%\fmfv{l=$a,,j$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$a,,0$,l.a=-55}{v1c}
\fmfv{l=$a,,0$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(-{2g_{v,a}\o\pi\ep}\)\(2g_{\A,a}-\sum_bg_{\A,b}\)\[\g^0\otimes\g^0\]\[\s^a\otimes\s_a\]$}
\label{fig:4ptsChi0ChiXArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}

==> 4pointsChiChiXY.tex <==
\centering
\begin{fmffile}{4ptsChiChiXY}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_plain}{v1a,v2a}
\fmf{dbl_plain}{v1b,v2b}
\fmfv{l=$b,,j$}{v1a}
\fmfv{l=$b,,j$}{v2a}
\fmfv{l=$a,,i$}{v1b}
\fmfv{l=$a,,i$}{v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
\caption{$\sum_{ab}\(g_{\A,a}g_{\A,b}\o\pi\ep\)\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]$
$+\sum_a\(-{g_{\A,a}^2\o\pi\ep}\)\[\g^j\otimes\g_j\]\[\id\otimes\id\]$}
%\label{fig:4ptSigmaSigmaNoX}
\label{fig:4ptChiChiNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_plain}{v1a,v2b}
\fmf{dbl_plain}{v1b,v2a}
\fmfv{l=$b,,j$}{v1a}
\fmfv{l=$b,,j$}{v2b}
\fmfv{l=$a,,i$}{v1b}
\fmfv{l=$a,,i$}{v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_{ab}\(g_{\A,a}g_{\A,b}\o\pi\ep\)\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]$
$+\sum_a\({g_{\A,a}^2\o\pi\ep}\)\[\g^j\otimes\g_j\]\[\id\otimes\id\]$}
\label{fig:4ptChiChiX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\
\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.40\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_plain}{v1c,v2c}
\fmf{photon,left,tension=0}{v1a,v1b}
\fmfv{l=$\m$}{v1b}
\fmfv{l=$\m$}{v1a}
\fmfv{l=$a$,l.a=-55}{v1c}
\fmfv{l=$a$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$a,,j$,l.a=-55}{v1c}
\fmfv{l=$a,,j$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\({16g_{\A,a}\mathpzc{g}^2\o3\pi^2(2N)\ep}\)\[\g^j\otimes\g_j\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}


==> 4pointsPhiChi0.tex <==
\centering
\begin{fmffile}{4ptsPhiChi0}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2a}
\fmf{dbl_wiggly}{v1b,v2b}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v2b}
\fmfv{l=$b$}{v1a}
\fmfv{l=$b$}{v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
\caption{
$
\sum_{a}\(g_{v,a}g_{t,a}\o2\pi\ep\)\[\g^j\otimes\g_j\]\[\id\otimes\id\]$
$+\sum_{ab}\(-{g_{v,a}g_{t,b}\o2\pi\ep}\)\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]
$}
%\label{fig:4ptSigmaSigmaNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\hspace{2mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2b}
\fmf{dbl_wiggly}{v1b,v2a}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v2a}
\fmfv{l=$b$}{v1a}
\fmfv{l=$b$}{v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\captionsetup{format=hang}
\caption{
$\sum_{a}\(g_{v,a}g_{t,a}\o2\pi\ep\)\[\g^j\otimes\g_j\]\[\id\otimes\id\]$
$+\sum_{ab}\({g_{v,a}g_{t,b}\o2\pi\ep}\)\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]
$}
%\label{fig:4ptSigmaSigmaX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_wiggly}{v1c,v2c}
\fmf{dbl_dashes,left,tension=0}{v1a,v1b}
%\fmfv{l=$a,,j$,l.a=-55}{v1c}
%\fmfv{l=$a,,j$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$a,,0$,l.a=-55}{v1c}
\fmfv{l=$a,,0$}{v2c}
\fmfv{l=$b$}{v1a}
\fmfv{l=$b$}{v1b}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(-{g_{v,a}\o\pi\ep}\)\(2g_{t,a}-\sum_bg_{t,b}\)\[\g^0\otimes\g^0\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\hspace{2mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmf{dbl_wiggly,left,tension=0}{v1a,v1b}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v1a}
\fmfv{l=$b$,l.a=-55}{v1c}
\fmfv{l=$b$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
%\fmfv{l=$a,,0$,l.a=-55}{v1c}
%\fmfv{l=$a,,0$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\({g_{t,a}\o\pi\ep}\)\(2g_{v,a}-\sum_bg_{v,b}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{8\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,30)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.8}{v1a,v1c,v1b}
\fmf{phantom,tension=.8}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{phantom,tension=0.7}{v1a,l1}
\fmf{phantom,tension=0.7}{v1b,r1}
\fmf{phantom,tension=0.7}{v1c,c1}
\fmf{phantom}{l1,l2,v2a}
\fmf{phantom}{r1,r2,v2b}
\fmf{phantom}{c1,c2,v2c}
\fmffreeze
\fmf{fermion}{i1,v1c}
\fmf{fermion}{v1c,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,c1}
\fmf{fermion}{c1,l2}
\fmf{fermion}{l2,r2}
\fmf{fermion}{r2,c1}
\fmf{photon}{l2,v2a}
\fmf{dbl_wiggly}{r2,v2b}
\fmfdot{v1c}
\fmfdot{v2a}
\fmfdot{v2b}
\fmfdot{c1}
\fmfdot{r2}
\fmfdot{l2}
\fmfv{l=$b$}{v1c}
\fmfv{l=$b$,l.a=0}{c1}
\fmfv{l=$a,,0$}{v2b}
\fmfv{l=$a,,0$}{r2}
\fmfv{l=$\m$}{l2}
\fmfv{l=$\m$}{v2a}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(-{4g_{t,a}g_{v,a}\mathpzc{g}^2\o\pi\ep}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
%\label{fig:FermLoopMassVerPotentialInt1}
\end{subfigure}
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}

==> 4pointsPhiChiXY.tex <==
\centering
\begin{fmffile}{4ptsPhiChiXY}
\scriptsize
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.50\textwidth}
\eq{2\times
\mff{
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2a}
\fmf{dbl_plain}{v1b,v2b}
\fmfv{l=$a,,j$}{v1b}
\fmfv{l=$a,,j$}{v2b}
\fmfv{l=$b$}{v1a}
\fmfv{l=$b$}{v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
\caption{
$\sum_a{g_{t,a}g_{\A,a}\o\pi\ep}\bigg\{
\[\id\otimes\id\]\[\id\otimes\id\]{-\[\g^0\otimes\g^0\]\[\id\otimes\id\]\bigg\}}$
$+\sum_{ab}{g_{t,a}g_{\A,b}\o\pi\ep}\sum_c\abs{\ep^{abc}}\bigg\{
-\[\id\otimes\id\]\[\s^c\otimes\s_c\]$
$+\[\g^0\otimes\g^0\]\[\s^a\otimes\s_a\]\bigg\}
$}
%\label{fig:4ptSigmaSigmaNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.49\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2b}
\fmf{dbl_plain}{v1b,v2a}
\fmfv{l=$a,,j$}{v1b}
\fmfv{l=$a,,j$}{v2a}
\fmfv{l=$b$}{v1a}
\fmfv{l=$b$}{v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\caption{
$\sum_a{g_{t,a}g_{\A,a}\o\pi\ep}\bigg\{
{-\[\id\otimes\id\]\[\id\otimes\id\]}{-\[\g^0\otimes\g^0\]\[\id\otimes\id\]}\bigg\}$ 
$+\sum_{ab} {g_{t,a}g_{\A,b}\o\pi\ep}\sum_c\abs{\ep^{abc}}
\bigg\{ {-\[\id\otimes\id\]}\[\s^c\otimes\s_c\]$ 
${-\[\g^0\otimes\g^0\]}\[\s^a\otimes\s_a\]\bigg\}
$}
%\label{fig:4ptSigmaSigmaX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmf{dbl_plain,left,tension=0}{v1a,v1b}
\fmfv{l=$a,,j$}{v1b}
\fmfv{l=$a,,j$}{v1a}
\fmfv{l=$b$,l.a=-55}{v1c}
\fmfv{l=$b$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
%\fmfv{l=$a,,0$,l.a=-55}{v1c}
%\fmfv{l=$a,,0$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(-{2g_{t,a}\o\pi\ep}\)\(2g_{\A,a}-\sum_bg_{\A,b}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\hspace{2mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{8\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,30)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.8}{v1a,v1c,v1b}
\fmf{phantom,tension=.8}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{phantom,tension=0.7}{v1a,l1}
\fmf{phantom,tension=0.7}{v1b,r1}
\fmf{phantom,tension=0.7}{v1c,c1}
\fmf{phantom}{l1,l2,v2a}
\fmf{phantom}{r1,r2,v2b}
\fmf{phantom}{c1,c2,v2c}
\fmffreeze
\fmf{fermion}{i1,v1c}
\fmf{fermion}{v1c,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,c1}
\fmf{fermion}{c1,l2}
\fmf{fermion}{l2,r2}
\fmf{fermion}{r2,c1}
\fmf{photon}{l2,v2a}
\fmf{dbl_plain}{r2,v2b}
\fmfdot{v1c}
\fmfdot{v2a}
\fmfdot{v2b}
\fmfdot{c1}
\fmfdot{r2}
\fmfdot{l2}
\fmfv{l=$b$}{v1c}
\fmfv{l=$b$,l.a=0}{c1}
\fmfv{l=$a,,j$}{v2b}
\fmfv{l=$a,,j$}{r2}
\fmfv{l=$\m$}{l2}
\fmfv{l=$\m$}{v2a}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a{4g_{t,a}g_{\A,a}\mathpzc{g}^2\o\pi\ep}\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
%\label{fig:FermLoopMassVerPotentialInt1}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}

==> 4pointsPhiPhi.tex <==
\centering
\begin{fmffile}{4ptsPhiPhi}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.49\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2a}
\fmf{dbl_dashes}{v1b,v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2a}
\fmfv{l=$b$}{v1b}
\fmfv{l=$b$}{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
\caption{$\sum_{ab}\(\m^{-2\ep}g_{t,a}g_{t,b}\o4\pi\ep\)\bigg\{\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]$
$-\d^{ab}\[\g^j\otimes\g_j\]\[\id\otimes\id\]\bigg\}$}
\label{fig:4ptPhiPhiNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.49\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2b}
\fmf{dbl_dashes}{v1b,v2a}
%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%\fmfkeep{suscept}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2b}
\fmfv{l=$b$}{v1b}
\fmfv{l=$b$}{v2a}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_{ab}\(\m^{-2\ep}g_{t,a}g_{t,b}\o4\pi\ep\)\bigg\{\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]$
$+\d^{ab}\[\g^j\otimes\g_j\]\[\id\otimes\id\]\bigg\}$}
\label{fig:4ptPhiPhiX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\
\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.49\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmf{dbl_dashes,left,tension=0}{v1a,v1b}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$b$}{v1a}
\fmfv{l=$b$}{v1b}
\fmfv{l=$a$,l.a=-55}{v1c}
\fmfv{l=$a$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a{\m^{-2\ep}g_{t,a}\o\pi\ep}\(2g_{t,a}-\sum_bg_{t,b}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
\label{fig:4ptPhiPhiVert}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.49\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmf{photon,left,tension=0}{v1a,v1b}
\fmfv{l=$\m$}{v1b}
\fmfv{l=$\m$}{v1a}
\fmfv{l=$a$,l.a=-55}{v1c}
\fmfv{l=$a$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(-{48\m^{-2\ep}g_{t,a}\mathpzc{g}^2\o\pi^2(4N)\ep}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
\label{fig:4ptsPhiPhiArc}
\end{subfigure}
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}

==> 4pointsPhiPhi2.tex <==
\centering
\begin{tabular{| c | c |}
\begin{fmffile}{4ptsPhiPhi2}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\hline
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2a}
\fmf{dbl_dashes}{v1b,v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2a}
\fmfv{l=$b$}{v1b}
\fmfv{l=$b$}{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
&
%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}[b]{0.49\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2b}
\fmf{dbl_dashes}{v1b,v2a}
%\fmfv{l=$q$,l.a=70,l.d=0.15w}{v2a}
%\fmfv{l=$\quad\;\; q+(1-s)p$,l.a=69,l.d=0.15w}{v2b}
%\fmfkeep{suscept}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2b}
\fmfv{l=$b$}{v1b}
\fmfv{l=$b$}{v2a}
\end{fmfgraph*}
}
\notag}
%\caption{$\sum_{ab}\(\m^{-2\ep}g_{t,a}g_{t,b}\o4\pi\ep\)\bigg\{\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]$
%$+\d^{ab}\[\g^j\otimes\g_j\]\[\id\otimes\id\]\bigg\}$}
%\label{fig:4ptPhiPhiX}
\\\hline
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
{$\sum_{ab}\(\m^{-2\ep}g_{t,a}g_{t,b}\o4\pi\ep\)\bigg\{\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]$
$-\d^{ab}\[\g^j\otimes\g_j\]\[\id\otimes\id\]\bigg\}$}
&
$\sum_{ab}\(\m^{-2\ep}g_{t,a}g_{t,b}\o4\pi\ep\)\bigg\{\sum_c\abs{\ep^{abc}}\[\g^j\otimes\g_j\]\[\s_c\otimes\s_c\]$
$+\d^{ab}\[\g^j\otimes\g_j\]\[\id\otimes\id\]\bigg\}$
\\\hline\hline
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}[b]{0.49\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmf{dbl_dashes,left,tension=0}{v1a,v1b}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$b$}{v1a}
\fmfv{l=$b$}{v1b}
\fmfv{l=$a$,l.a=-55}{v1c}
\fmfv{l=$a$}{v2c}
\end{fmfgraph*}
}
\notag}
%\caption{$\sum_a{\m^{-2\ep}g_{t,a}\o\pi\ep}\(2g_{t,a}-\sum_bg_{t,b}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptPhiPhiVert}
%\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
&
%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}[b]{0.49\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmf{photon,left,tension=0}{v1a,v1b}
\fmfv{l=$\m$}{v1b}
\fmfv{l=$\m$}{v1a}
\fmfv{l=$a$,l.a=-55}{v1c}
\fmfv{l=$a$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\end{fmfgraph*}
}
\notag}
%\caption{$\sum_a\(-{48\m^{-2\ep}g_{t,a}\mathpzc{g}^2\o\pi^2(4N)\ep}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsPhiPhiArc}
%\end{subfigure}
%\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\\ \hline
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
$\sum_a{\m^{-2\ep}g_{t,a}\o\pi\ep}\(2g_{t,a}-\sum_bg_{t,b}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$
&
$\sum_a\(-{48\m^{-2\ep}g_{t,a}\mathpzc{g}^2\o\pi^2(4N)\ep}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$
\\\hline
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}{4ptsPhiPhi2}
\end{tabular}

==> 4pointsSigmaChi0.tex <==
\centering
\begin{fmffile}{4ptsSigmaChi0}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2a}
\fmf{dbl_wiggly}{v1b,v2b}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
\caption{
$\sum_a\({ g_sg_{v,a}\o2\pi\ep}\)\[\g^j\otimes\g_j\]\[\s^a\otimes\s_a\]
$}
%\label{fig:4ptSigmaSigmaNoX}
\label{fig:4ptSigmaChi0NoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2b}
\fmf{dbl_wiggly}{v1b,v2a}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\caption{
$\sum_a\({ g_sg_{v,a}\o2\pi\ep}\)\[\g^j\otimes\g_j\]\[\s^a\otimes\s_a\]
$}
\label{fig:4ptSigmaChi0X}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_wiggly}{v1c,v2c}
\fmf{dashes,left,tension=0}{v1a,v1b}
%\fmfv{l=$a,,j$,l.a=-55}{v1c}
%\fmfv{l=$a,,j$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$a,,0$,l.a=-55}{v1c}
\fmfv{l=$a,,0$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(-{ g_sg_{v,a}\o\pi\ep}\)\[\g^0\otimes\g^0\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1c,v2c}
\fmf{dbl_wiggly,left,tension=0}{v1a,v1b}
\fmfv{l=$a,,0$}{v1b}
\fmfv{l=$a,,0$}{v1a}
%\fmfv{l=$a,,j$,l.a=-55}{v1c}
%\fmfv{l=$a,,j$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
%\fmfv{l=$a,,0$,l.a=-55}{v1c}
%\fmfv{l=$a,,0$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\[\id\otimes\id\]\[\id\otimes\id\]\({ g_s\o\pi\ep}\sum_ag_{v,a}\)$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}

==> 4pointsSigmaChiXY.tex <==
\centering
\begin{fmffile}{4ptsSigmaChiXY}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2a}
\fmf{dbl_plain}{v1b,v2b}
\fmfv{l=$a,,j$}{v1b}
\fmfv{l=$a,,j$}{v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
\captionsetup{format=hang,justification=centering}
\centering
\caption{
$\sum_a\( g_sg_{\A,a}\o\pi\ep\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$
$+\sum_a\(-{ g_sg_{\A,a}\o\pi\ep}\)\[\g^0\otimes\g^0\]\[\s^a\otimes\s_a\]
$}
%\label{fig:4ptSigmaSigmaNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2b}
\fmf{dbl_plain}{v1b,v2a}
\fmfv{l=$a,,j$}{v1b}
\fmfv{l=$a,,j$}{v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\caption{
$\sum_a\(-{ g_sg_{\A,a}\o\pi\ep}\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$
$+\sum_a\(-{ g_sg_{\A,a}\o\pi\ep}\)\[\g^0\otimes\g^0\]\[\s^a\otimes\s_a\]
$}
%\label{fig:4ptSigmaSigmaX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\\\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1c,v2c}
\fmf{dbl_plain,left,tension=0}{v1a,v1b}
\fmfv{l=$a,,j$}{v1b}
\fmfv{l=$a,,j$}{v1a}
%\fmfv{l=$a,,j$,l.a=-55}{v1c}
%\fmfv{l=$a,,j$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
%\fmfv{l=$a,,0$,l.a=-55}{v1c}
%\fmfv{l=$a,,0$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\(-{2 g_s\o\pi\ep}\sum_ag_{\A,a}\)\[\id\otimes\id\]\[\id\otimes\id\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}

==> 4pointsSigmaPhi.tex <==
\centering
\begin{fmffile}{4ptsSigmaPhi}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.48\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2a}
\fmf{dashes}{v1b,v2b}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
\notag}
%\vspace{8mm}
\caption{
$\sum_a\(-{g_sg_{t,a}\o2\pi\ep}\)\[\g^j\otimes\g_j\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptSigmaSigmaNoX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1a,v2b}
\fmf{dashes}{v1b,v2a}
\fmfv{l=$a$}{v1a}
\fmfv{l=$a$}{v2b}
\fmfdot{v1a}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\caption{
$\sum_a\({g_sg_{t,a}\o2\pi\ep}\)\[\g^j\otimes\g_j\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptSigmaSigmaX}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%
\\\vspace{8mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1c,v2c}
\fmf{dbl_dashes,left,tension=0}{v1a,v1b}
\fmfv{l=$a$}{v1b}
\fmfv{l=$a$}{v1a}
%\fmfv{l=$a,,j$,l.a=-55}{v1c}
%\fmfv{l=$a,,j$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\[\id\otimes\id\]\[\id\otimes\id\]\({g_s\o\pi\ep}\sum_ag_{t,a}\)$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{2\times
\mff{
\scriptsize
\begin{fmfgraph*}(35,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=1.55}{v1a,v1c,v1b}
\fmf{phantom,tension=1.55}{v2a,v2c,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion,label=$q$,label.side=left}{v1a,v1b}
\fmf{fermion}{v1a,v1c}
\fmf{fermion}{v1c,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{plain}{v2a,v2c}
\fmf{plain}{v2c,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dbl_dashes}{v1c,v2c}
\fmf{dashes,left,tension=0}{v1a,v1b}
%\fmfv{l=$b,,j$}{v1b}
%\fmfv{l=$b,,j$}{v1a}
%\fmfv{l=$a,,j$,l.a=-55}{v1c}
%\fmfv{l=$a,,j$}{v2c}
\fmfdot{v1a}
\fmfdot{v1c}
\fmfdot{v1b}
\fmfdot{v2c}
\fmfv{l=$a$,l.a=-55}{v1c}
\fmfv{l=$a$}{v2c}
\end{fmfgraph*}
}
\notag}
\caption{$\sum_a\(g_sg_{t,a}\o\pi\ep\)\[\id\otimes\id\]\[\s^a\otimes\s_a\]$}
%\label{fig:4ptsSigmaPhotonArc}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}
%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}

==> FullFluxRenorm.tex <==
\begin{fmffile}{FullFluxRenorm}
\fmfset{dot_size}{1.5thick}
\fmfset{arrow_len}{3mm}%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(60,15)
\fmfpen{thin}
\fmfstraight
\fmfleft{i1}
\fmfright{o1}
\fmf{photon}{i1,v1}
\fmf{phantom}{v1,v2}
\fmf{phantom,tension=0.6}{v2,v3}
\fmf{phantom}{v3,v4}
\fmf{photon}{v4,o1}
\fmffreeze
\fmf{fermion,right}{v3,v4}
\fmf{fermion,right}{v4,v3}
\fmf{fermion,right}{v1,v2}
\fmf{fermion,right}{v2,v1}
\fmf{dbl_plain}{v2,vC,v3}
\fmfv{decor.shape=hexagon,decor.filled=shaded,decor.size=7mm}{vC}
\fmfdot{v1,v2,v3,v4}
\end{fmfgraph*}
}
\notag}
\caption{}
\label{fig:3LoopIntgB}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(60,15)
\fmfpen{thin}
\fmfstraight
\fmfleft{i1}
\fmfright{o1}
\fmf{photon}{i1,v1}
\fmf{phantom}{v1,v2}
\fmf{phantom,tension=0.6}{v2,v3}
\fmf{phantom}{v3,v4}
\fmf{photon}{v4,o1}
\fmffreeze
\fmf{fermion,right}{v3,v4}
\fmf{fermion,right}{v4,v3}
\fmf{fermion,right}{v1,v2}
\fmf{fermion,right}{v2,v1}
\fmf{dbl_plain}{v2,vC,v3}
\fmfv{decor.shape=hexagon,decor.filled=empty,decor.size=7mm}{vC}
\fmfdot{v1,v2,v3,v4}
\end{fmfgraph*}
}
\notag}
\caption{}
\label{fig:3LoopIntgE}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}

==> InternalFermionLoop.tex <==
\centering
\begin{fmffile}{InternalFermionLoop}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\centering
\eq{
\mfff{
\scriptsize
\begin{fmfgraph*}(20,17)
\fmfpen{thin}
\fmfstraight
\fmfleft{i1,i2,i3}
\fmfright{o1,o2,o3}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=0.6}{v2a,v2b}
\fmf{phantom}{v2b,o2}
\fmf{phantom}{i1,v1a}
\fmf{phantom,tension=0.6}{v1a,v1b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{i3,v3a}
\fmf{phantom,tension=0.6}{v3a,v3b}
\fmf{phantom}{v3b,o3}
\fmffreeze
\fmf{photon}{i2,v2a}
\fmf{fermion,label=$q$,label.side=left}{v1b,v2a}
\fmf{fermion,label=$q+k$,label.side=left}{v3b,v1b}
\fmf{fermion,label=$q$,label.side=left}{v2a,v3b}
\fmf{photon}{v1b,o1}
\fmf{dbl_dots}{v3b,o3}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v3b}
\fmfv{label=$\mu$,l.a=90}{v2a}
\fmfv{label=$\nu$}{v1b}
\end{fmfgraph*}
}
\notag}
%\vspace{4mm}
\caption{}
\label{fig:IntFermionLoop1}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.45\textwidth}
\centering
\eq{
\mfff{
\scriptsize
\begin{fmfgraph*}(20,17)
\fmfpen{thin}
\fmfstraight
\fmfleft{i1,i2,i3}
\fmfright{o1,o2,o3}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=0.6}{v2a,v2b}
\fmf{phantom}{v2b,o2}
\fmf{phantom}{i1,v1a}
\fmf{phantom,tension=0.6}{v1a,v1b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{i3,v3a}
\fmf{phantom,tension=0.6}{v3a,v3b}
\fmf{phantom}{v3b,o3}
\fmffreeze
\fmf{photon}{i2,v2a}
\fmf{fermion,label=$q$,label.side=right}{v2a,v1b}
\fmf{fermion,label=$q-k$,label.side=right}{v1b,v3b}
\fmf{fermion,label=$q$,label.side=right}{v3b,v2a}
\fmf{dbl_dots}{v1b,o1}
\fmf{photon}{v3b,o3}
\fmfdot{v2a}
\fmfdot{v1b}
\fmfdot{v3b}
\fmfv{label=$\mu$,l.a=90}{v2a}
\fmfv{label=$\nu$}{v3b}
\end{fmfgraph*}
}
%\notag
}
%\vspace{4mm}
\caption{}
%\label{fig:IntFermionLoop2}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}
\vspace{5mm}

==> counterTerm.tex <==
\begin{fmffile}{counterTerm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}[b]{0.45\textwidth}
\eq{
\mff{
\small
\begin{fmfgraph*}(35,20)
\fmfcurved
\fmfleft{i1,i3,i2}
\fmfright{o1,o3,o2}
\fmflabel{$\mu,r,\a$}{i3}
\fmflabel{$\nu,s,\b$}{o3}
\fmf{phantom}{i1,x1,o1}
\fmf{phantom}{o2,x2,i2}
\fmfv{decor.size=1.5mm,decor.shape=square,decor.filled=gray50}{i3}
\fmfv{decor.size=1.5mm,decor.shape=square,decor.filled=gray50}{o3}
\fmffreeze
\fmf{fermion,right=0.6,label={\scriptsize$q+p$}}{i3,o3}
%\fmf{fermion,left=0.3,tension=0.3,label={\scriptsize$q$}}{x1,i3}
%\fmf{fermion,left=0.3,tension=0.3,label={\scriptsize$q+k$}}{o3,x1}
\fmf{fermion,right=0.3,tension=0.3,label={\scriptsize$q$}}{o3,x2}
\fmf{fermion,right=0.3,tension=0.3,label={\scriptsize$q$}}{x2,i3}
\fmfv{decor.shape=hexagram,decor.filled=shaded}{x2}
\end{fmfgraph*}}
\notag\vspace{5mm}}
\caption{The star indicates the counter term from }
\label{fig:currentLoopCounter}
%\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{fmffile}
\vspace{5mm}

==> fluxVertex.tex <==
\centering
\begin{fmffile}{fluxVertex}
\fmfset{dot_size}{1.5thick}
\fmfset{arrow_len}{3mm}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%% INTERNAL PHOTON LINES %%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(20,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
%\fmf{phantom,tension=1.3}{v1a,v1b}
%\fmf{phantom,tension=1.3}{v2a,v2b}
\fmf{phantom}{v1a,o1}
\fmf{phantom}{v2a,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion}{i1,v1a}
%%\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1a,o1}
\fmf{fermion}{i2,v2a}
%\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2a,o2}
\fmf{dbl_plain}{v1a,vC,v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmffreeze
\fmfv{decor.shape=hexagon,decor.filled=shaded,decor.size=7mm}{vC}
\end{fmfgraph*}}
=
\mff{
\scriptsize
\begin{fmfgraph*}(25,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2a}
\fmf{photon}{v1b,vC1}
\fmf{phantom,tension=1.8}{vC1,vC2}
\fmf{photon}{vC2,v2b}
\fmffreeze
%\fmfdot{vC1}
%\fmfdot{vC2}
\fmfpoly{shade}{vC1,vb,vC2,vt}
\fmfv{label=$0$,l.a=0}{vC1}
\fmfv{label=$0$,l.a=0}{vC2}
\fmfv{l=0}{v1b}	
\fmfv{l=0}{v2b}
\fmfdot{v1a}
\fmfdot{v1b}
\fmfdot{v2a}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
+
\mff{
\scriptsize
\begin{fmfgraph*}(25,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2b}
\fmf{photon}{v1b,vC1}
\fmf{phantom,tension=2.2}{vC1,vC2}
\fmf{photon}{vC2,v2a}
\fmffreeze
%\fmfdot{vC1}
%\fmfdot{vC2}
\fmfpoly{shade}{vC1,vb,vC2,vt}
\fmfv{label=$0$,l.a=0}{vC1}
\fmfv{label=$0$,l.a=180}{vC2}
\fmfv{l=0}{v1b}	
\fmfv{l=0}{v2a}
\fmfdot{v1a}
\fmfdot{v1b}
\fmfdot{v2a}
\fmfdot{v2b}
\end{fmfgraph*}
}
+
\mff{
\scriptsize
\begin{fmfgraph*}(25,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1b,v2b}
\fmf{photon}{v1a,vC1}
\fmf{phantom,tension=1.8}{vC1,vC2}
\fmf{photon}{vC2,v2a}
\fmffreeze
%\fmfdot{vC1}
%\fmfdot{vC2}
\fmfpoly{shade}{vC1,vb,vC2,vt}
\fmfv{label=$0$,l.a=0}{vC1}
\fmfv{label=$0$,l.a=0}{vC2}
\fmfv{l=0}{v1a}	
\fmfv{l=0}{v2a}
\fmfdot{v1a}
\fmfdot{v1b}
\fmfdot{v2a}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
+
\mff{
\scriptsize
\begin{fmfgraph*}(25,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1b,v2a}
\fmf{photon}{v1a,vC1}
\fmf{phantom,tension=2.2}{vC1,vC2}
\fmf{photon}{vC2,v2b}
\fmffreeze
%\fmfdot{vC1}
%\fmfdot{vC2}
\fmfpoly{shade}{vC1,vb,vC2,vt}
\fmfv{label=$0$,l.a=180}{vC1}
\fmfv{label=$0$,l.a=0}{vC2}
\fmfv{l=0}{v1a}	
\fmfv{l=0}{v2b}
\fmfdot{v1a}
\fmfdot{v1b}
\fmfdot{v2a}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
%\vspace{5mm}
\caption{}
\label{fig:gBVert}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%% INTERNAL PHOTON LINES %%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{\textwidth}
\eq{
\mff{
\scriptsize
\begin{fmfgraph*}(20,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
%\fmf{phantom,tension=1.3}{v1a,v1b}
%\fmf{phantom,tension=1.3}{v2a,v2b}
\fmf{phantom}{v1a,o1}
\fmf{phantom}{v2a,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
%\fmf{fermion}{i1,v1a}
%%\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1a,o1}
\fmf{fermion}{i2,v2a}
%\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2a,o2}
\fmf{dbl_plain}{v1a,vC,v2a}
\fmfdot{v1a}
\fmfdot{v2a}
\fmffreeze
\fmfv{decor.shape=hexagon,decor.filled=empty,decor.size=7mm}{vC}
\end{fmfgraph*}}
=
\mff{
\scriptsize
\begin{fmfgraph*}(25,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2a}
\fmf{photon}{v1b,vC1}
\fmf{phantom,tension=1.8}{vC1,vC2}
\fmf{photon}{vC2,v2b}
\fmffreeze
%\fmfdot{vC1}
%\fmfdot{vC2}
\fmfpoly{empty}{vC1,vb,vC2,vt}
\fmfv{label=$i$,l.a=0}{vC1}
\fmfv{label=$j$,l.a=0}{vC2}
\fmfv{l=$i$}{v1b}	
\fmfv{l=$j$}{v2b}
\fmfdot{v1a}
\fmfdot{v1b}
\fmfdot{v2a}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
+
\mff{
\scriptsize
\begin{fmfgraph*}(25,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1a,v2b}
\fmf{photon}{v1b,vC1}
\fmf{phantom,tension=2.2}{vC1,vC2}
\fmf{photon}{vC2,v2a}
\fmffreeze
%\fmfdot{vC1}
%\fmfdot{vC2}
\fmfpoly{empty}{vC1,vb,vC2,vt}
\fmfv{label=$i$,l.a=0}{vC1}
\fmfv{label=$j$,l.a=180}{vC2}
\fmfv{l=$i$}{v1b}	
\fmfv{l=$j$}{v2a}
\fmfdot{v1a}
\fmfdot{v1b}
\fmfdot{v2a}
\fmfdot{v2b}
\end{fmfgraph*}
}
+
\mff{
\scriptsize
\begin{fmfgraph*}(25,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1b,v2b}
\fmf{photon}{v1a,vC1}
\fmf{phantom,tension=1.8}{vC1,vC2}
\fmf{photon}{vC2,v2a}
\fmffreeze
%\fmfdot{vC1}
%\fmfdot{vC2}
\fmfpoly{empty}{vC1,vb,vC2,vt}
\fmfv{label=$i$,l.a=0}{vC1}
\fmfv{label=$j$,l.a=0}{vC2}
\fmfv{l=$i$}{v1a}	
\fmfv{l=$j$}{v2a}
\fmfdot{v1a}
\fmfdot{v1b}
\fmfdot{v2a}
\fmfdot{v2b}
%\fmfkeep{suscept}
\end{fmfgraph*}}
+
\mff{
\scriptsize
\begin{fmfgraph*}(25,20)
\fmfpen{thin}
\fmfstraight
\fmfleft{i2,i1}
\fmfright{o2,o1}
%\fmflabel{$\mu$}{i1}
%\fmf{phantom,tension=2}{i1,o1}
%\fmffreeze
\fmf{phantom}{i1,v1a}
\fmf{phantom}{i2,v2a}
\fmf{phantom,tension=.6}{v1a,v1b}
\fmf{phantom,tension=.6}{v2a,v2b}
\fmf{phantom}{v1b,o1}
\fmf{phantom}{v2b,o2}
\fmffreeze
\fmf{fermion}{i1,v1a}
\fmf{fermion}{v1a,v1b}
\fmf{fermion}{v1b,o1}
\fmf{fermion}{i2,v2a}
\fmf{fermion}{v2a,v2b}
\fmf{fermion}{v2b,o2}
\fmf{dashes}{v1b,v2a}
\fmf{photon}{v1a,vC1}
\fmf{phantom,tension=2.2}{vC1,vC2}
\fmf{photon}{vC2,v2b}
\fmffreeze
%\fmfdot{vC1}
%\fmfdot{vC2}
\fmfpoly{empty}{vC1,vb,vC2,vt}
\fmfv{label=$i$,l.a=180}{vC1}
\fmfv{label=$j$,l.a=0}{vC2}
\fmfv{l=$i$}{v1a}	
\fmfv{l=$j$}{v2b}
\fmfdot{v1a}
\fmfdot{v1b}
\fmfdot{v2a}
\fmfdot{v2b}
\end{fmfgraph*}
}
\notag}
\caption{}
\label{fig:gEVert}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%


\end{fmffile}

==> headers.tex <==
\usepackage[margin=0.7in]{geometry}
%\usepackage[square,numbers]{natbib}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{verbatim}
\usepackage{braket}
\usepackage{enumitem}
\DeclareGraphicsRule{*}{mps}{*}{}
\usepackage{feynmp}
\unitlength = 1mm
\usepackage{math tools} %\Aboxed{ } draws boxes around '&' in align
\usepackage{dsfont} %gives the ``double stroke 1" I like to use for the identity \mathds{}
\usepackage{mathrsfs} %give very curly math script. I use it for \hilb=\mathscr{H}, Hilbert space H 
%\usepackage{pbox} %for adding boxes not in equations
%\usepackage{undertilde} %for a tilde under a letter/symbol, such as in a simapprox
\usepackage{parskip} %removes automatic indenting of paragraphs
\usepackage{mathabx} %has sun symbol \Sun, (also: \Earth, \Moon)
\usepackage{multirow}
\usepackage{arydshln} %\hdashline
\usepackage{lscape}%\begin{landscape} -- \end{landscape} makes landscape pages
\usepackage{slashed}%gives Dirac slash -- \slashed(\partial) -- I make a shortcut below
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor} %coloured text
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it} %lower case cursive -- ie. \mathpzc{g}


% allows line spacing changes
\usepackage{setspace}
\setstretch{1.06} % changes spacing

% From Subir's manuscript (doubles removed)
\usepackage{amssymb,mathrsfs,bm,xspace,soul} 
\usepackage{graphicx}  
\usepackage{color} 

\usepackage[colorlinks=true]{hyperref} 
\hypersetup{
    bookmarks=true,         % show bookmarks bar?
    unicode=false,          % non-Latin characters 
    pdftoolbar=true,        % show Acrobat
    pdfmenubar=true,        % show Acrobat 
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdftitle={My title},    % title
    pdfauthor={Author},     % author
    pdfsubject={Subject},   % subject of the document
    pdfcreator={Creator},   % creator of the document
    pdfproducer={Producer}, % producer of the document
    pdfkeywords={keyword1} {key2} {key3}, % list of keywords
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=magenta, %red,          % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    filecolor=magenta,      % color of file links
    urlcolor=cyan           % color of external links
} 

%\usepackage{chngcntr} %counter
%\counterwithin{figure}{section}

% Special math character shortcuts


%\mathcal shortcuts
\newcommand{\ord}{\mathcal{O}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\hamk}{\mathcal{H}}
\newcommand{\bcX}{\boldsymbol{\mathcal{X}}}
\newcommand{\bcW}{\boldsymbol{\mathcal{W}}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\V}{\mathcal{V}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\D}{\mathcal{D}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\E}{\mathcal{E}}

%\mathscr shortcuts
\newcommand{\hilb}{\mathscr{H}}

%\mathbf shortcuts
%\newcommand{\vn}{{\mathbf{n}}}
%\newcommand{\vk}{{\mathbf{k}}}
%\newcommand{\vr}{{\mathbf{r}}}
%\newcommand{\vQ}{{\mathbf{Q}}}
%\newcommand{\vK}{{\mathbf{K}}}
%\newcommand{\vq}{{\mathbf{q}}}
%\newcommand{\vp}{{\mathbf{p}}}
%\newcommand{\vx}{{\mathbf{x}}}
%\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vn}{{\boldsymbol{n}}}
\newcommand{\vk}{{\boldsymbol{k}}}
\newcommand{\vr}{{\boldsymbol{r}}}
\newcommand{\vQ}{{\boldsymbol{Q}}}
\newcommand{\vK}{{\boldsymbol{K}}}
\newcommand{\vq}{{\boldsymbol{q}}}
\newcommand{\vp}{{\boldsymbol{p}}}
\newcommand{\vx}{{\boldsymbol{x}}}
\newcommand{\vy}{{\boldsymbol{y}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\hx}{\hat{\mathbf{x}}}
\newcommand{\hy}{\hat{\mathbf{y}}}

% Unit vectors - bold with hats
\newcommand{\hvx}{\mathbf{\hat{x}}}
\newcommand{\hvy}{\mathbf{\hat{y}}}
\newcommand{\hvm}{\boldsymbol{\hat{\mu}}}
\newcommand{\hvn}{\mathbf{\hat{n}}}
\newcommand{\bchi}{\hat{\bb{\chi}}}

% Other math shortcuts
\newcommand{\vphi}{{\varphi}}
\newcommand{\ham}{\hat{H}}
\newcommand{\tphi}{\tilde{\phi}}
\newcommand{\bpsi}{\bar{\psi}}
\newcommand{\bz}{\bar{z}}
\newcommand{\tr}{\text{tr}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\sd}[1]{\slashed{#1}}

% Math commands - General
\newcommand{\final}{\comment} %comment out figures that take a long time to load
\renewcommand{\o}{\over}
\newcommand{\eq}[1]{\begin{align}#1\end{align}}
\newcommand{\eql}[1]{\begin{align}#1\end{align}}

% Brackets
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\newcommand{\abs}[1]{\left| #1 \right|}

% Spacing and newlines in math mode
\newcommand{\nt}{\notag\\}
\newcommand{\tnl}{\\[1.5ex]}

% Math typesetting commands
\let\spt\mathcal
%\renewcommand{\v}{\boldsymbol}%
\let\v\mathbf
\newcommand{\ti}{\tilde}
\newcommand{\bb}{\boldsymbol}
\newcommand{\ph}{\phantom}

%Greek letters
\newcommand{\ep}{\epsilon}
\newcommand{\vep}{\varepsilon}
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\renewcommand{\d}{\delta}
\newcommand{\g}{\gamma}
\newcommand{\n}{\nu}
\newcommand{\m}{\mu}
\renewcommand{\t}{\tau}
\newcommand{\s}{\sigma}
\newcommand{\w}{\omega}
\renewcommand{\th}{\theta}
\newcommand{\vth}{\vartheta}
\newcommand{\vph}{\varphi}
\newcommand{\lam}{\lambda}
\renewcommand{\r}{\rho}
\newcommand{\Lam}{\Lambda}
\renewcommand{\k}{\kappa}

% Math Symbols
\let\ptl\partial
\renewcommand{\dag}{\dagger}
\newcommand{\ninfty}{{-\infty}}
\newcommand{\fr}{\mathcal{F}}
\newcommand{\id}{\mathds{1}}
\newcommand{\Zt}{\mathds{Z}_2}
\newcommand{\Z}{\mathds{Z}}
\renewcommand\Re{\operatorname{\mathfrak{Re}}}
\renewcommand\Im{\operatorname{\mathfrak{Im}}}
\def\dbar{{\mathchar'26\mkern-12mu d}} %d-slash using in thermodynamics

% Arrows
\newcommand{\ua}{\uparrow}
\newcommand{\da}{\downarrow}
%\renewcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}

% Hyperbolic trig functions
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}
\DeclareMathOperator{\arcsinh}{arcsinh}

% Jacobi theta functions
\newcommand{\jthetac}[2]{\vartheta\begin{bmatrix}#1\\#2\end{bmatrix}}
\newcommand{\jThetac}[2]{\Theta\begin{bmatrix}#1\\#2\end{bmatrix}}

%Raise box for Feynman diagram
\newcommand{\mf}[1]{\raisebox{-0.4\height}{\hbox{ {#1}}}}
\newcommand{\mff}[1]{\raisebox{-0.49\height}{\hbox{ {#1}}}}

%Allow margin change for part of page
\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist 

% Itemize shortcut
\newcommand{\lst}[1]{\begin{itemize}#1\end{itemize}}
\newcommand{\pt}{\item}

%table of contents
\usepackage{tocloft} 
% \cftpagenumbersoff{chapters}
\addtocontents{toc}{\cftpagenumbersoff{chapter}}
\addtocontents{toc}{\cftpagenumbersoff{section}}

\setlist[enumerate]{leftmargin=*}

%fancy overbar
%\newsavebox\myboxA
%\newsavebox\myboxB
%\newlength\mylenA
%
%\newcommand*\xoverline[2][0.75]{%
%    \sbox{\myboxA}{$\m@th#2$}%
%    \setbox\myboxB\null% Phantom box
%    \ht\myboxB=\ht\myboxA%
%    \dp\myboxB=\dp\myboxA%
%    \wd\myboxB=#1\wd\myboxA% Scale phantom
%    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
%    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
%    \addtolength\mylenA{-\the\wd\myboxB}%
%    \ifdim\wd\myboxB<\wd\myboxA%
%       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
%    \else
%        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
%    \fi}
%    \makeatother

